LT-mapper: A Modular Framework for LiDAR-based Lifelong Mapping

Long-term 3D map management is a fundamental capability required by a robot to reliably navigate in the non-stationary real-world. This paper develops open-source, modular, and readily available LiDAR-based lifelong mapping for urban sites. This is achieved by dividing the problem into successive subproblems: multi-session SLAM (MSS), high/low dynamic change detection, and positive/negative change management. The proposed method leverages MSS and handles potential trajectory error; thus, good initial alignment is not required for change detection. Our change management scheme preserves efficacy in both memory and computation costs, providing automatic object segregation from a large-scale point cloud map. We verify the framework's reliability and applicability even under permanent year-level variation, through extensive real-world experiments with multiple temporal gaps (from day to year).

==> src/alg/alg_ltmap.tex <==
\setlength{\textfloatsep}{0.1cm}

\begin{algorithm}[t!]

    \SetAlgoLined

    \footnotesize

    \SetKwInOut{Input}{input}
    \SetKwInOut{Output}{output}
    \Input
    {
        $r$, $\mathcal{P}_{t_{N}}$, $[$LD$^{t_{c+1}}_{t_{c}}$$]$$_{t_c = 1, ..., N-1}$
    }
    \Output
    {
        $\hat{\mathcal{P}}_{t_{r}}$
    }

    $\mathcal{P}_{est} = \mathcal{P}_{t_{N}}$; \\

    \For{$c = N-1, N-2, ..., r+1, r$}
    {
        $\mathcal{P}_{est}$ $=$ $\mathcal{P}_{est}$ $\odot$ LD$^{t_c}_{t_{c+1}}$;    
    }

    $\hat{\mathcal{P}}_{t_{r}} = \mathcal{P}_{est}$;

    \vspace{1mm}

    \caption
    {
        LT-map: N-session change composition
    }

    \label{alg:ltmap}

\end{algorithm}

\setlength{\textfloatsep}{0.1cm}


==> src/alg/alg_ltremovert.tex <==
\setlength{\textfloatsep}{0.1cm}
% \setlength{\floatsep}{0.1cm}

\begin{algorithm}[t!]

    \SetAlgoLined
  
    % \scriptsize
    \footnotesize
  
    \SetKwInOut{Input}{input}
    \SetKwInOut{Output}{output}
    \Input
    {
        \{$\mathcal{P}_{C}$\}, \{$\mathcal{P}_{Q}$\}, ${}^{C'}\mathcal{G}_{C}^{*}$, ${}^{C'}\mathcal{G}_{Q}^{*}$
    }
    \Output
    {
        \{$\tilde{\mathcal{P}}_{C}$\}, \{\text{LD}$^{Q}_{C}$\}
    }

    \vspace{1mm}

    \nonl \_ 1. Remove high dynamic points \hrulefill\\ 
    $($\{$\tilde{\mathcal{P}}_{C}$\}, $\tilde{\mathcal{M}}_{C}$$)$ $=$ removert$\big($${\mathcal{M}}_{C}$ $\vert$ \{$\mathcal{P}_{C}$\}, ${}^{C'}\mathcal{G}_{C}^{*}$$\big)$; \\
    $($\{$\tilde{\mathcal{P}}_{Q}$\}, $\tilde{\mathcal{M}}_{Q}$$)$ $=$ removert$\big($${\mathcal{M}}_{Q}$ $\vert$ \{$\mathcal{P}_{Q}$\}, ${}^{C'}\mathcal{G}_{Q}^{*}$$\big)$; \\
    \vspace{1.5mm}

    \nonl \_ 2. Detect low dynamic changes \hrulefill\\ 
    \{$\mathcal{P}^{PD}_{C}$\} $=$ knnSetDiff$\big($\{$\tilde{\mathcal{P}}_{Q}$\}, ${}^{C'}\mathcal{G}_{Q}^{*}$ $\vert$ $\tilde{\mathcal{M}}_{C}$$\big)$; \\
    \{$\mathcal{P}^{ND}_{C}$\} $=$ knnSetDiff$\big($\{$\tilde{\mathcal{P}}_{C}$\}, ${}^{C'}\mathcal{G}_{C}^{*}$ $\vert$ $\tilde{\mathcal{M}}_{Q}$$\big)$; \\
    \vspace{1.5mm}

    \nonl \_ 3. Occlusion check to filter strong LD \hrulefill\\ 
    \{$\tilde{\mathcal{P}}^{PD}_{C}$\} $=$ removert$\big($$\mathcal{M}^{PD}_{C}$ $\vert$ \{$\tilde{\mathcal{P}}_{Q}$\}, ${}^{C'}\mathcal{G}_{Q}^{*}$$\big)$;\\ 
    \{$\tilde{\mathcal{P}}^{ND}_{C}$\} $=$ iremovert$\big($$\mathcal{M}^{ND}_{C}$ $\vert$ \{$\tilde{\mathcal{P}}_{Q}$\}, ${}^{C'}\mathcal{G}_{Q}^{*}$$\big)$;\\
    \vspace{1.5mm}

    \nonl \_ 4. Return by packing a LD struct: (PD, ND) \hrulefill\\
    \uIf{isToMakeMetaMap \text{/* see Fig. 9. */} }{
        \{\text{LD}$^{Q}_{C}$\} $=$ \{$($PD: $\tilde{\mathcal{P}}^{PD}_{C}$, ND: $\tilde{\mathcal{P}}^{ND}_{C}$$)\};$
    }
    \Else{
        \{\text{LD}$^{Q}_{C}$\} $=$ \{$($PD: $\mathcal{P}^{PD}_{C}$, ND: $\tilde{\mathcal{P}}^{ND}_{C}$$)\};$
    }
    \vspace{1mm}

    \caption
    {
        LT-removert: HD removal, LD detection
    }

    \label{alg:ltremovert}

\end{algorithm}

\setlength{\textfloatsep}{0.1cm}


==> src/alg/alg_ltslam.tex <==
\setlength{\textfloatsep}{0.1cm}
\begin{algorithm}[t!]

    % \SetAlgoShortEnd

    % \scriptsize
    \footnotesize

    \SetKwInOut{Input}{input}
    \SetKwInOut{Output}{output}
    \Input
    {
        $\mathcal{S}_{C}$, $\mathcal{S}_{Q}$
    }
    \Output
    {
        ${}^{C'}\mathcal{G}_{C}^{*}$, ${}^{C'}\mathcal{G}_{Q}^{*}$
    }

    \vspace{1mm}

    % loadSessions([$\mathcal{S}_{C}$, $\mathcal{S}_{Q}$]); \\
    loadSessions; \hl{READIBILITY? DIAGRAM INSTEAD?} \\

    \vspace{1mm}

    initializeFactorGraph; assignAnchorNodes; \\

    \vspace{1mm}

    constructScanContextLoopDetectors; \\
    detectIntersessionLoopsUsingScanContext; \\
    addFactorsUsingICP; optimizeGraph; \\

    \vspace{1mm}

    updateKeyframePoseEstimates; \\
    detectIntersessionLoopsUsingRadiusSearch; \\
    addFactorsUsingICP; optimizeGraph; \\

    \vspace{1mm}

    saveCoframeTransformedGraphs;

    \vspace{1mm}

    \caption
    {
        LT-SLAM: multi-session alignment
    }

    \label{alg:ltslam}

\end{algorithm}

\setlength{\textfloatsep}{0.1cm}


==> src/exp-abnormal.tex <==
%-------------------------------------------------------%
%-------------------------------------------------------%
% \subsection{Abnormal Change Detection}
% \label{sec:abnormal}


% + Memory Efficiency 

% \figref{fig:memory}

==> src/exp-eff.tex <==
%--------------------------------%
%--------------------------------%
\subsection{Efficiency}
\label{sec:effi}

\subsubsection{Efficient Change Detection with Arbitrary Time Gap} 

\textbf{Time costs and memory usages}


\subsubsection{Efficient Change Detection with Arbitrary Time Gap} 

\figref{fig:memory}

We saved the storage, but if we want to access a certain time of snapshot.
We can roll-back the version. 



==> src/fig/fig_change_composition.tex <==
%FIGURE
\begin{figure}[!t]
  \centering

  \subfigure[ QL]{%
  \includegraphics[width=0.97\columnwidth, trim = 0 60 0 40, clip]{figs/spacer/changecompqual}
      \label{fig:changecompositionql}
  } 
  \\
  \subfigure[ QT ]{%
  \includegraphics[width=0.97\columnwidth, trim = 0 80 0 20, clip]{figs/spacer/changecompquant}
      \label{fig:changecompositionqt}
  }

  \caption
  {
    Change Composition 
  }

  \label{fig:changecomposition}

\end{figure}
%FIGURE


==> src/fig/fig_diff_sensitivity.tex <==
%FIGURE
\begin{figure}[!t]
  \centering

  \includegraphics[width=0.98\columnwidth]{figs/ltremovert/sensitivity}
  \vspace{-3mm}
  \caption
  {
    Different LD results under two extreme k-NN sensitivity cases. Due to the unavoidable SLAM error, the building walls were not exactly registered (yellow boxes). This would provoke false LD changes when we use a highly sensitive k-NN threshold. On the contrary, using low sensitivity would miss true small changes, such as cars (magenta boxes). This example is from the scene in \figref{fig:cover}. 
  }

  \label{fig:sensitivity}

  \vspace{-3mm}

\end{figure}
%FIGURE


==> src/fig/fig_ld_cases.tex <==
%FIGURE
\begin{figure}[!t]
  \centering

  \includegraphics[width=0.75\columnwidth, trim = 25 0 -15 0, clip]{figs/ltremovert/ldcases}
  \vspace{-3mm}
  \caption
  {
    The exemplars (\texttt{A}) and (\texttt{B}) from \texttt{DCC 01} and \texttt{02} of \texttt{MulRan} dataset. (\texttt{A}) includes occlusion where no points exist (red dotted box), due to the construction wall (blue-lined box). The wall disappears later, revealing the ground points in (\texttt{B}). Selection of central session as \texttt{A} and query session as \texttt{B} will be \texttt{Case 1}; the reversed case is \texttt{Case 2}. The left column is the naive ND and PD points from the set difference operation. The right column shows accepted ND and PD points after weak ND point validation. In \texttt{Case 1}, red ND points were mostly removed while adding entire blue PD points. In \texttt{Case 2}, some ground points are occluded and marked as ND. In the right column, only strong ND (red) points are removed, and weak ND points are reverted (e.g., ground points marked with gray).
  }
  \label{fig:ldcases}

  \vspace{-3mm}

\end{figure}
%FIGURE


==> src/fig/fig_lifelong.tex <==
\begin{figure*}[!t]
  \centering

  % \subfigure[ \texttt{ParkingLot} map evolution: normal and solid ver.]{%
  % \includegraphics[width=0.97\textwidth, trim = 0 0 0 0, clip]{figs/spacer/lifelong}
  %     \label{fig:lifelongqual1}
  % } 
  % \\
  % \subfigure[ \texttt{ParkingLot} with strong \ac{PD} ]{%
  % \includegraphics[width=0.97\textwidth, trim = 0 0 0 0, clip]{figs/spacer/lifelong}
  %     \label{fig:lifelongqual2}
  % }

  \includegraphics[width=0.98\textwidth, trim = 0 -20 0 -20, clip]{figs/spacer/lifelong}
  \caption
  {
    Lifelong mapping examaple. \texttt{ParkingLot} map evolution: normal and solid ver.
  }
  \label{fig:lifelongqual}

  % \vspace{-5mm}

\end{figure*}

%FIGURE



==> src/fig/fig_ltslam_pipeline.tex <==
%FIGURE
\begin{figure}[!b]
  \centering
  \vspace{-4mm}

  \includegraphics[width=0.85\columnwidth, trim = 6 0 -10 0, clip]{figs/ltslam/ltslampipeline.pdf}
  \vspace{-2mm}
  \caption
  {
    The pipeline of LT-SLAM.
  }

  \label{fig:ltslampipeline}
  % \vspace{-4mm}
\end{figure}
%FIGURE


==> src/fig/fig_ltslam_qual.tex <==
\begin{figure*}[!t]
  \centering
  \captionsetup{font=footnotesize}

  \resizebox{.95\textwidth}{!}{
  \centering
  \subfigure[ { \texttt{KAIST} sequences of \texttt{MulRan} dataset } ]{%
  \includegraphics[width=0.40\textwidth, trim = 0 0 0 0, clip]{figs/ltslam/ltslam-ql-a-v2}
      \label{fig:ltslamqual1}
  } \ \ \
  \subfigure[ { \texttt{LT-ParkingLot} dataset } ]{%
  \includegraphics[width=0.52\textwidth, trim = 0 -10 0 0, clip]{figs/ltslam/ltslam-ql-b}
      \label{fig:ltslamqual2}
  }
  }

  % \vspace{-2mm}
  \caption
  {
    \subref{fig:ltslamqual1} The baseline \texttt{LO} (red) is obtained by LIO-SAM's \cite{shan2020lio} odometry without loop closures. \subref{fig:ltslamqual2} The left is an aerial view of \texttt{LT-ParkingLot} dataset. The middle plot shows different sessions' trajectories acquired at different dates in the dataset. While covering the same area, trajectories were not aligned, as they occupy their own coordinates. The right plot shows that \textbf{LT-SLAM} simultaneously estimates between-session offsets while reducing the drifts. Thus, multiple sessions can be aligned in a shared world coordinate for change detection. The height differences are imposed for clear visualization.
  }
  \label{fig:ltslamqual}

  \vspace{-5mm}

\end{figure*}
%FIGURE


==> src/fig/fig_memory.tex <==
\begin{figure*}[!t]
  \centering

  % \subfigure[ \texttt{ParkingLot} map evolution: normal and solid ver.]{%
  % \includegraphics[width=0.97\textwidth, trim = 0 0 0 0, clip]{figs/spacer/lifelong}
  %     \label{fig:lifelongqual1}
  % }
  % \\
  % \subfigure[ \texttt{ParkingLot} with strong \ac{PD} ]{%
  % \includegraphics[width=0.97\textwidth, trim = 0 0 0 0, clip]{figs/spacer/lifelong}
  %     \label{fig:lifelongqual2}
  % }

  \includegraphics[width=0.99\textwidth, trim = 0 0 -3 0, clip]{figs/ltmap/memory}
  \vspace{-3mm}
  \caption
  {
    \textbf{LT-mapper} can detect unexpected changes without human intervention. (a) Places of \figref{fig:cover} in \texttt{KAIST 01} and \texttt{KAIST 02} are revisited in \texttt{KAIST 04} (b) The changes between \texttt{02} and \texttt{01} are small (the yellow line, average \unit{18}{\%} compared to all snapshots). (c) The LD change ratio is increased compared to (b) after keyframe 650 (red box), whereas the ratio remains the same (green box). (d) Ratio difference of (b) and (c). The abnormal change increase (i.e., new construction wall in \figref{fig:cover}) is particularly vivid in this difference of ratios. 
  }
  \label{fig:memory}

  \vspace{-4mm}

\end{figure*}

%FIGURE


==> src/fig/fig_method_loop.tex <==
%FIGURE
\begin{figure}[!t]
  \centering

  \includegraphics[width=0.96\columnwidth]{figs/spacer/method1}
  \caption
  {
      TODO 
  }
  \label{fig:methodloop}
\end{figure}
%FIGURE


==> src/fig/fig_method_removert.tex <==
%FIGURE
\begin{figure}[!t]
  \centering

  \includegraphics[width=0.95\columnwidth]{figs/spacer/method2}
  \caption
  {
      TODO 
  }
  \label{fig:methodremovert}

  \vspace{-3mm}

\end{figure}
%FIGURE


==> src/fig/fig_mstraj.tex <==
%FIGURE
\begin{figure}[!t]
  \centering

  \includegraphics[width=0.8\columnwidth]{figs/spacer/mstraj}
  \caption
  {
      TODO 
  }
  \label{fig:mstraj}
\end{figure}
%FIGURE


==> src/fig/format/fig_single.tex <==
%FIGURE
\begin{figure}[!t]
    \centering
  
    \includegraphics[width=0.99\columnwidth]{figs/airmap}
    \caption
    {
      The dataset trajectories overlaid on each aerial map. The first column shows \texttt{KAIST 03 (MulRan)} and \texttt{Riverside 02 (MulRan)}, followed by \texttt{Oxford Radar RobotCar}, the \texttt{Sejong} sequence in \texttt{MulRan}, and \texttt{Pangyo (NAVER LABS)}. The magenta boxes on the right show the wide roads in the \texttt{Pangyo} sequence of the \texttt{NAVER LABS} dataset. The total length of each sequence and their characteristics are summarized in \tabref{tab:dataset}.
    }
    \label{fig:datasetviz}
\end{figure}
%FIGURE
  

==> src/fig/table_datasets.tex <==
%FIGURE
\begin{figure}[!t]
  \centering

  \includegraphics[width=0.98\columnwidth]{figs/spacer/table}
  \caption
  {
      TODO this is actually Table later  
  }
  \label{fig:dataset}
\end{figure}
%FIGURE


==> src/related_work.tex <==

\section{Related Works}
\label{sec:related}

%---------------------------------------------------%
\subsubsection{Multi-session SLAM}

Registration between scans may be vulnerable, failing even with small and partial structural variance. Thus, as claimed in \cite{kim2010multiple, orbatlas19}, jointly smoothing the multiple sessions can improve query-to-map localization performance despite potential motion drift. For example, DPG-SLAM \cite{walcott2012dynamic} aligned multiple sessions' SE(2) trajectories using pose graph optimization before conducting change detection. Similar to \cite{walcott2012dynamic} but extending it to 3D, our proposed method supports robust inter-session global localization \cite{kim2018scan} and improved loop-closures \cite{kim2010multiple, ila2009information} without a priori information.

% for efficiency ex glc but beyond our interest. to relieve the big graph pgo computation issue as in \cite{walcott2012dynamic}, we introduce a Markov-like sequential map update will be seen in \secref{sec:ltmap}


%---------------------------------------------------%
\subsubsection{3D Change Detection}

For change detection between well-aligned maps, a set difference operation can be conducted via extracting map-to-map complements \cite{ambrucs2014meta, wellhausen2017reliable}. Otherwise, visibility-based scan-to-map discrepancy comparison \cite{pomerleau2014long, schauer2018peopleremover, gskim-2020-iros, palazzolo2018fast} has been a popular choice, because of the small covisible volume and inherent localization errors. Removert \cite{gskim-2020-iros} leveraged range images of multiple window sizes while removing with finer windows followed by reverting with coarser matchings. However, their approach have not treated high and low dynamic points separately. Also, Removert was restricted to a single session while the proposed \textbf{LT-removert} handles multi-session scenarios by combining the map-to-map complements and the visibility-based scan-to-map methods.
% However, they have not treated high and low dynamic points separately.

%---------------------------------------------------%
\subsubsection{Lifelong Map Representation}

Map representation is also important for map maintenance in long-term mapping. The example of the representation varies from traditional occupancy grid maps \cite{tipaldi2013lifelong, sun2018recurrent, banerjee2019lifelong} to frequency domain representation \cite{krajnik2017fremen}. For change detection in 3D environments, dealing with a direct raw 3D point cloud may be preferred over the occupancy map-based ones. \citeauthor{pomerleau2014long} \cite{pomerleau2014long} proposed to update 3D point-wise static probability via the Bayesian model. In this method and \cite{ambrucs2014meta}, a query scan is assumed to be well localized within the map. This may be an unrealistic assumption in the real-world, where each scan possesses its associated frame with potential \ac{SLAM} error. With respect to the atomic map update unit, our approach is similar to \cite{ambrucs2014meta}, which showed delta-based updates. Unlike them, we manage an atomic update at a keyframe level. This contributes to systems scalability, without being restricted to a fixed global frame \cite{pomerleau2014long} or room level \cite{ambrucs2014meta}.

% but not SLAM integrated
% For visual sensor, ORBSLAM-Atlas \cite{orbatlas19} operates a single unified sparse 3D point cloud map from multiple-sessions. For LiDAR sensor, \

%---------------------------------------------------%
% \noindent \textbf{Long-term Map Management.}


%---------------------------------------------------%
% Summary
%---------------------------------------------------%
\subsubsection{Modular Design of Lifelong Mapper}

The abovementioned single modules have been developed individually, whereas a unified system has hardly been discovered for LiDAR. DPG-SLAM \cite{walcott2012dynamic} combined the full modules but was constrained in 2D space, and functionalities of robust loop detection and change detection in 3D point clouds were missing. \cite{pomerleau2014long} was also equipped with entire modules, except for \ac{MSS}. Also, it is a limitation of \cite{pomerleau2014long} that a point's lifespan is managed within a global frame, whereas our \textbf{LT-map} manages the pointwise changes per-place level in local coordinates. This means that our map management can be readily decoupled from \textbf{LT-SLAM} (i.e., independent of the map nodes' pose adjustments over time).
% The benefits of our approach will be introduced in \secref{sec:ltremovert}.


==> src/tab/param.tex <==
% \setlength{\textfloatsep}{0.1cm}

\begin{table}[!b]
    \vspace{2mm}

    \centering % centering table
    {\scriptsize % tiny, footnotesize, small

    \begin{tabular}{c c c c c} % creating 10 columns
    \toprule

    Module & Submodule & Parameter  & Value
    \\ [0.5ex]

    \hline \\[-2ex]

    Common & Map resolution & Voxel size & \unit{0.05}{m}$^{3}$ \\

    \hline \\[-2ex]

                              &                               & ROI   & \unit{[0, 80]}{m}, \unit{[0, 360]}{\degree}  \\[0ex]
                              &                               & Descriptor shape   & 20$\cross$60  \\[-2ex]
    \raisebox{2.5ex}{LT-SLAM} & \raisebox{2.5ex}{Scan Context}& Distance threshold & 0.3 \\

    \hline\\[-1.9ex]
                                  &                               & Vertical FOV          & [$-25$\degree, $25$\degree]  \\[-.3ex]
                                  &                               & Removing pixel size   & 0.4\degree$\cross$ 0.4\degree  \\[-2ex]
    \raisebox{2.5ex}{LT-removert}   & \raisebox{2ex}{Removert}      & Reverting pixel size  & 0.45\degree$\cross$ 0.45\degree \\[-0.1ex]
    % \raisebox{3ex}{LT-removert}   &  k-NN                         & $(k, r)$: high / low  & (2, 0.2) / (5, 1.0) \\

    \bottomrule

    \end{tabular}
    }

    \vspace{2mm}

    \caption
    {
        Parameters of \textbf{LT-mapper}
    } % title name of the table

    \label{tab:param}
    \vspace{-2mm}

\end{table}

% \setlength{\textfloatsep}{0.1cm}

